Flocking-Segregative Swarming Behaviors using Gibbs Random Fields

This paper presents a novel approach that allows a swarm of heterogeneous robots to produce simultaneously segregative and flocking behaviors using only local sensing. These behaviors have been widely studied in swarm robotics and their combination allows the execution of several complex tasks, ranging from surveillance and reconnaissance, to search and rescue, to transport, and to foraging. Although there are several works in the literature proposing different strategies to achieve these behaviors, to the best of our knowledge, this paper is the first to propose an algorithm that emerges simultaneously behaviors and do not rely on global information or communication. Our approach consists of modeling the swarm as a Gibbs Random Field (GRF) and using appropriate potential functions to reach segregation, cohesion and consensus on the velocity of the swarm. Simulations and proof-of-concept experiments using real robots are presented to evaluate the performance of our methodology in comparison to some of the state-of-the-art works that tackle segregative behaviors.

==> sections/temp.tex <==
\subsection{Applications} % or Other behaviors
As we state,  the combination of segregative and flocking behaviors allows the execution of several complex tasks. Further, we intend to deal with such tasks using the methodology presented in this work. For instance, we aim to investigate swarm transportation and shape-formation in the context of heterogeneity groups. Fig.~\ref{fig:segregationexp} shows an initial step toward to shape-formation. 

\begin{figure}[h]
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0001.png}
		\caption{$n=0$}
		\label{fig:rangerobots}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0042.png}
		\caption{$n=200$}
		\label{fig:rangegroups}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0322.png}
		\caption{$n=1600$}
		\label{fig:shapeformation}
	\end{subfigure}%
	\caption{Initial steps toward shape-formation task. Virtual points with heterogeneous attraction are placed in the environment so that robots of a specific type are attracted, resulting in the formation of structures. A video is available at \url{https://youtu.be/uJs0fwiQHIc}.} % footnote
	\label{fig:segregationexp}
\end{figure}



\begin{algorithm}[t]
\caption{Calculate robot $i$ velocity at time $t+1$}\label{alg:metropolis}
\Procedure{Update}{$\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)}$} 
 \State $\mathbf{V}^{(0)} \gets \mathbf{v_i}^{(t)}$, \Comment{Set of velocities} 
 \State $\mathbf{U}^{(0)} \gets H(\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)})$, \Comment{Set of potential energies} 
 \For{$k \gets 1$ to $\mathcal{I}$}
%  \State $\mathbf{v}_{prev} \gets \mathbf{V}$(end),  \Comment{Get the last element of $\mathbf{V}$} 
%  \State $\mathbf{u}_{prev} \gets \mathbf{U}$(end),  \Comment{Get the last element of $\mathbf{U}$} 
 \State $\bar{\mathbf{v}} \gets N(\mathbf{v_i}^{(t)}, \mathbf{\Sigma})$,    \Comment{Gaussian sampling} 
 \State $\bar{\mathbf{u}} \gets  H(\mathbf{q_i}^{(t)}, \bar{\mathbf{v}})$,
 \State $\Delta E \gets \bar{\mathbf{u}} - \mathbf{U}^{(k-1)}$,      \Comment{Potential energy variation}
 \State $g \gets exp(-\Delta E)$,   \Comment{Compute the gibbs energy}
 \State $r \gets \mathcal{U}(0, 1)$,   \Comment{Uniform sampling}
 \If{$(\Delta E < 0) \lor (r < g)$ } \Comment{Sample is accepted}
    \State $\mathbf{V}^{(k)} \gets \bar{\mathbf{v}}$,
    \State $\mathbf{U}^{(k)} \gets \bar{\mathbf{u}}$,
    \Else \Comment{Sample is rejected}
    \State $\mathbf{V}^{(k)} \gets  {\mathbf{V}^{(k-1)}}$,
    \State $\mathbf{U}^{(k)} \gets  {\mathbf{U}^{(k-1)}}$,
    \EndIf
 \EndFor
%  \State $\mathbf{V} \gets \mathbf{V}^{(j,...,\mathcal{I})}$, \Comment{Reject the first j velocities}
 \State $\mathbf{v_i}^{(t+1)} \gets  (\mathbf{V}^q + ...+\mathbf{V}^\mathcal{I})/(\mathcal{I}-q)$, \Comment{Average velocity}
 \State \textbf{return} $\mathbf{v_i}^{(t+1)}$
\EndProcedure
\end{algorithm}


